Teaching Programming to Novices Using the codeBoot Online Environment

Teaching programming to novices is best done with tools with simpler user interfaces than professional IDEs that are tailored for experienced programmers. In a distance learning situation it is also important to have a development environment that is easy to explain and use, and that integrates well with the variety of course material used (slides, homework, etc). In this paper we give an experience report on teaching programming with codeBoot, an online programming environment we designed specifically for novices.

==> eptcsdata.tex <==
\providecommand{\firstpage}{44}
\providecommand{\publicationstatus}{P. Achten \& E. Machkasova  (Eds.): Trends in\\
Functional Programming in Education (TFPIE) 2021/22
\\
EPTCS 363, 2022, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.363.3}{10.4204/EPTCS.363.3}}
\pdfoutput=1

